Detecting and Summarizing GUI Changes in Evolving Mobile Apps

Mobile applications have become a popular software development domain in recent years due in part to a large user base, capable hardware, and accessible platforms. However, mobile developers also face unique challenges, including pressure for frequent releases to keep pace with rapid platform evolution, hardware iteration, and user feedback. Due to this rapid pace of evolution, developers need automated support for documenting the changes made to their apps in order to aid in program comprehension. One of the more challenging types of changes to document in mobile apps are those made to the graphical user interface (GUI) due to its abstract, pixel-based representation. In this paper, we present a fully automated approach, called GCAT, for detecting and summarizing GUI changes during the evolution of mobile apps. GCAT leverages computer vision techniques and natural language generation to accurately and concisely summarize changes made to the GUI of a mobile app between successive commits or releases. We evaluate the performance of our approach in terms of its precision and recall in detecting GUI changes compared to developer specified changes, and investigate the utility of the generated change reports in a controlled user study. Our results indicate that GCAT is capable of accurately detecting and classifying GUI changes - outperforming developers - while providing useful documentation.

==> macro.tex <==


\usepackage{amssymb}
\usepackage{ifthen}

\makeatletter

% this  is a easy way to add and highlight new text  ...
% just comment in/out the \tnew macro ..

\newcommand*{\img}[1]{%
    \raisebox{-.3\baselineskip}{%
        \includegraphics[
        height=\baselineskip,
        width=\baselineskip,
        keepaspectratio,
        ]{#1}%
    }%
}

\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\pagenumbering{arabic}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}

\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }

\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\etals}{\textit{et al.'s}\xspace}
\newcommand{\aka}{\textit{a.k.a.}\xspace}	


\newcommand\TODO[1]{{\color{red} \nb{TODO}{#1}}}
\newcommand\KEVIN[1]{{\color{blue} \nb{KEVIN}{#1}}}
\newcommand\JOHN[1]{{\color{blue}\nb{JOHN}{#1}}}
\newcommand\DENYS[1]{{\color{blue}\nb{DENYS}{#1}}}
\newcommand\GEORGE[1]{{\color{blue}\nb{GEORGE}{#1}}}
\newcommand\CODY[1]{{\color{blue}\nb{CODY}{#1}}}

\newcommand\NEW[1]{\nb{NEW}{#1}}






==> tab/subjects.tex <==
\begin{table}[]
\centering
\caption{Subject Applications and Versions used in Quantitative and Qualitative Empirical Studies}
\label{tab:subjects}
\scriptsize
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{App name}   & \textbf{App Versions} & \textbf{LoC Old} & \textbf{LoC New} & \textbf{\# Downloads} \\ \hline
FastHub Libre       & 3.0.0 $\mid$ 4.6.2         & 88444            & 152107           & 100,000+              \\ \hline
Authorizer          & 0.2.4 $\mid$ 0.2.5         & 46984            & 47667            & 100+                  \\ \hline
AnyMemo             & 10.9 $\mid$ 10.9.993       & 44847            & 44093            & 100,000+              \\ \hline
Gear Shift          & 0.9.96 $\mid$ 1.0.5   & 39637            & 42246            & N/A                   \\ \hline
Book Catalougue     & 3.7 $\mid$ 3.8.1           & 31607            & 31946            & 100,000+              \\ \hline
Easer               & 0.4.9 $\mid$ 0.5.5.3       & 23928            & 30149            & N/A                   \\ \hline
Calendar            & 3.1.0 $\mid$ 3.3.2         & 22326            & 23412            & 500,000+              \\ \hline
ServeStream         & 0.4.6 $\mid$ 0.4.8         & 19878            & 20086            & 100,000+              \\ \hline
SkyTube             & 2.7.0 $\mid$ 2.8.0         & 17670            & 20425            & N/A                   \\ \hline
Flym                & 1.9.0 $\mid$ 1.9.1         & 17384            & 17359            & 50,000+               \\ \hline
LnkShortener        & 1.0.2 $\mid$ 1.1.2         & 16464            & 30196            & 50+                   \\ \hline
fwknop2             & 1.0 $\mid$ 1.2.3           & 15540            & 20810            & 1,000+                \\ \hline
SysLog              & 2.0.2 $\mid$ 2.1.2         & 13340            & 13141            & 100,000+              \\ \hline
Equate              & 1.4 $\mid$ 1.6             & 12706            & 13924            & 10,000+               \\ \hline
SGit                & 1.3.0 $\mid$ 1.3.2         & 11097            & 11863            & 50,000+               \\ \hline
Simple Weather      & 4.1 $\mid$ 5.3.2           & 10210            & 10662            & 10,000+               \\ \hline
Earmouse            & 1.2.2 $\mid$ 1.2.3         & 6022             & 6114             & 500+                  \\ \hline
Simple Dilbert      & 4.3 $\mid$ 4.5             & 3659             & 3841             & N/A                   \\ \hline
Bullseye            & 0.1 $\mid$ 0.3             & 3272             & 3185             & N/A                   \\ \hline
Fon                 & 1.5.1 $\mid$ 1.5.2         & 3151             & 3152             & 100,000+              \\ \hline
Sound Recorder      & 1.2.5 $\mid$ 1.3.0         & 3025             & 3211             & 5,000+                \\ \hline
Sensors20SC         & 0.1.0 $\mid$ 0.3.0         & 2670             & 2637             & N/A                   \\ \hline
Currency            & 1.0 $\mid$ 1.5             & 2546             & 5559             & N/A                   \\ \hline
Simple-Calculator   & 2.0.0 $\mid$ 3.1.2         & 2484             & 2801             & 10,000+               \\ \hline
StageFever          & 1.0.8 $\mid$ 1.0.9         & 2461             & 1971             & N/A                   \\ \hline
Counter             & 13 $\mid$ 18               & 2012             & 2880             & 100,000+              \\ \hline
Draw                & 1.14 $\mid$ 2.3.0          & 1993             & 2288             & 100,000+              \\ \hline
App Launcher        & 2.0.0 $\mid$ 3.1.1         & 1807             & 1781             & 10,000+               \\ \hline
Dumbphone Asst. & 0.4 $\mid$ 0.5             & 1566             & 1600             & N/A                   \\ \hline
Snotepad            & 1.0 $\mid$ 1.2.1           & 1406             & 1479             & N/A                   \\ \hline
\end{tabular}
\end{table}
